All-sky Medium Energy Gamma-ray Observatory: Exploring the Extreme Multimessenger Universe

The All-sky Medium Energy Gamma-ray Observatory (AMEGO) is a probe class mission concept that will provide essential contributions to multimessenger astrophysics in the late 2020s and beyond. AMEGO combines high sensitivity in the 200 keV to 10 GeV energy range with a wide field of view, good spectral resolution, and polarization sensitivity. Therefore, AMEGO is key in the study of multimessenger astrophysical objects that have unique signatures in the gamma-ray regime, such as neutron star mergers, supernovae, and flaring active galactic nuclei. The order-of-magnitude improvement compared to previous MeV missions also enables discoveries of a wide range of phenomena whose energy output peaks in the relatively unexplored medium-energy gamma-ray band.

==> coauthors_with_email.tex <==
%\emph{This section will be removed before submission and pasted into the textbox on the WP submission form. Please add your name following the format  ``Name, Affiliation, Email, Name, Affiliation, Email...''}


Alexander van der Horst, George Washington University, ajvanderhorst@email.gwu.edu,

Alberto Dominguez, Universidad Complutense de Madrid, alberto@gae.ucm.es,

Alexander Moiseev, CRESST/NASA/GSFC, alexander.a.moiseev@nasa.gov,

Alexandre Marcowith, Laboratoire Univers et Particules de Montpellier, alexandre.marcowith@umontpellier.fr,

Alice Harding, NASA/GSFC, alice.k.harding@nasa.gov,

Amy Lien, CRESST/NASA/GSFC, amy.y.lien@nasa.gov,

Andrea Giuliani, Instituto Nazionale di Astrofisica,andrea.giuliani@inaf.it,

Andrew Inglis, CUA/NASA/GSFC, andrew.inglis@nasa.gov,

Stefano Ansoldi, University of Udine, ansoldi@fulbrightmail.org,

Antonio Stamerra, Instituto Nazionale di Astrofisica, antonio.stamerra@inaf.it,

Antonios Manousakis, Copernicus Astronomical Center, antonism@camk.edu.pl,

Andy Strong, Max Planck Institute for Extraterrestrial Physics, aws@mpe.mpg.de,

Cosimo Bambi, Fudan University, bambi@fudan.edu.cn,


Barbara Patricelli, University of Pisa & INFN, barbara.patricelli@pi.infn.it, 

Matthew Baring, Rice University, baring@rice.edu, 

Juan Abel Barrio, Universidad Complutense de Madrid, barrio@gae.ucm.es, 

Denis Bastieri, University of Padova & INFN Padova, bastieri@pd.infn.it, 

Brian Fields, University of Illinois, bdfields@illinois.edu, 

John Beacom, The Ohio State University, beacom.7@osu.edu, 

Volker Beckmann, CNRS/IN2P3, beckmann@in2p3.fr 

Wlodek Bednarek, Uniwersytet Łódzki, bednar@uni.lodz.pl, 

Bindu Rani, CRESST/NASA/GSFC, bindu.rani@nasa.gov,

Steven Boggs, University of California San Diego, seboggs@ucsd.edu,

Aleksey Bolotnikov, Brookhaven National Lab, bolotnik@bnl.gov,

S. Brad Cenko, NASA/GSFC, brad.cenko@nasa.gov,

Jim Buckley, Washington University in St. Louis, buckley@physics.wustl.edu,

Brian Grefenstette, California Institute of Technology, bwgref@srl.caltech.edu,

Michelle Hui, NASA/MSFC, c.m.hui@nasa.gov,

Carlotta Pittori, ASI Space Science Data Center, carlotta.pittori@ssdc.asi.it, 

Chanda Prescod-Weinstein, University of New Hampshire, chanda.prescod-weinstein@unh.edu,

Chris Shrader, CRESST/NASA/GSFC, chris.r.shrader@nasa.gov,

Christian Gouiffes, Commissariat á l'Energie Atomique, christian.gouiffes@cea.fr,

Carolyn Kierans, NPP/NASA/GSFC, carolyn.a.kierans@nasa.gov,

Colleen Wilson-Hodge, NASA/MSFC, colleen.wilson@nasa.gov,

Filippo D'Ammando, Istituto di Radioastronomia & INAF, dammando@ira.inaf.it,

Daniel Castro, Harvard-Smithsonian CfA, daniel.castro@cfa.harvard.edu,

Daniel Kocveski, NASA/MSFC, daniel.kocevski@nasa.gov,

Dario Gasparrini, ASI Space Science Data Center, dario.gasparrini@ssdc.asi.it,

David Thompson, NASA/GSFC, david.j.thompson@nasa.gov,

David Williams, University of California Santa Cruz, daw@ucsc.edu,

Alessandro De Angelis, University of Padova & INFN Padova,deangelis.alessandro@gmail.com,

Denis Bernard, CNRS/IN2P3, denis.bernard@in2p3.fr, 

Seth Digel, SLAC National Accelerator Laboratory, digel@slac.stanford.edu,

Daniel Morcuende, Universidad Complutense de Madrid, dmorcuen@ucm.es,

Eric Charles, SLAC National Accelerator Laboratory, echarles@slac.stanford.edu,

Elisabetta Bissaldi, INFN Sezione di Bari, Elisabetta.Bissaldi@ba.infn.it,

Elizabeth Hays, NASA/GSFC, elizabeth.a.hays@nasa.gov, 

Elizabeth Ferrara, CRESST/NASA/GSFC, elizabeth.c.ferrara@nasa.gov,

Enrico Bozzo, Université de Genève, enrico.bozzo@unige.ch,

Eric Grove, Naval Research Lab, eric.grove@nrl.navy.mil,

Eric Wulf, Naval Research Lab, eric.wulf@nrl.navy.mil,

Eugenio Bottacini, University of Padova, eugenio.bottacini@unipd.it,

Ezio Caroli, Instituto Nazionale di Astrofisica, ezio.caroli@inaf.it,

Fabian Kislat, University of New Hampshire, fabian.kislat@unh.edu, 

Foteini Oikonomou, European Southern Observatory, foikonom@eso.org, 

Francesco Giordano, INFN Sezione di Bari, francesco.giordano@ba.infn.it, 

Francesco Longo, University of Trieste & INFN, francesco.longo@trieste.infn.it,

Chris Fryer, Los Alamos National Lab, fryer@lanl.gov, 

Yasushi Fukazawa, Hiroshima University, fukazawa@astro.hiroshima-u.ac.jp,

Markos Georganopoulos, University of Maryland Baltimore County, georgano@umbc.edu,

Georgia De Nolfo, NASA/GSFC, georgia.a.denolfo@nasa.gov,

Giacomo Vianello, Stanford University, giacomov@slac.stanford.edu,

Gottfried Kanbach, Max Planck Institute for Extraterrestrial Physics, gok@mpe.mpg.de, 

George Younes, George Washington University, gyounes@email.gwu.edu,

Harsha Blumer, West Virginia University, harshablumer1@gmail.com,

Dieter Hartmann, Clemson University, hdieter@clemson.edu,

Margarita Hernanz, Universitat de Barcelona, hernanz@ieec.uab.es, 

Hiromitsu Takahashi, Hiroshima University, hirotaka@astro.hiroshima-u.ac.jp,

Hui Li, Los Alamos National Lab, hli@lanl.gov,

Ivan Agudo, Instituto de Astrofísica de Andalucía, iagudo@iaa.es, 

Igor Moskalenko, Stanford University, imos@stanford.edu,

Inga Stumke, Universitetet i Bergen, inga.strumke@uib.no,

Isabelle Grenier, Commissariat á l'Energie Atomique, isabelle.grenier@cea.fr, 

Jacob Smith, CRESST/NASA/GSFC, jacob.umd.work@gmail.com, 

James Rodi, IAPS-INAF, james.rodi@iaps.inaf.it, 

Jeremy Perkins, NASA/GSFC, jeremy.s.perkins@nasa.gov, 

Joseph Gelfand, New York University, jg168@nyu.edu,

Jamie Holder, University of Delaware, jholder@physics.udel.edu,

Jurgen Knodlseder, L'Observatoire Midi-Pyrénées, jknodlseder@irap.omp.eu,

Joachim Kopp, Die Johannes Gutenberg-Universität Mainz, jkopp@uni-mainz.de, 

Jean-Philippe Lenain, CNRS/IN2P3, jlenain@in2p3.fr,

José-Manuel Álvarez, Centro De Láseres Pulsados, jmalvarez@clpu.es, 

Jessica Metcalfe, Argonne National Lab, jmetcalfe@anl.gov,

John Krizmanic, CRESST/NASA/GSFC, john.f.krizmanic@nasa.gov,

John B. Stephen, INAF/IASF Bologna, john.stephen@inaf.it, 

Jack Hewitt, University of North Florida, john.w.hewitt@unf.edu,

John Mitchell, NASA/GSFC, john.w.mitchell@nasa.gov,

Pat Harding, Los Alamos National Lab, jpharding@lanl.gov, 

John Tomsick, University of California Berkeley, jtomsick@ssl.berkeley.edu,

Judith Racusin, NASA/GSFC, judith.racusin@nasa.gov,

Justin Finke, Naval Research Lab, justin.finke@nrl.navy.mil,

Oleg Kargaltsev, George Washington University, kargaltsev@email.gwu.edu,

Alexei V. Klimenko, Los Alamos National Lab, klimenko@lanl.gov,

Henric Krawczynsiki, Washington University in St. Louis, krawcz@wuphys.wustl.edu,

Karl Smith, Los Alamos National Lab, ksmith@lanl.gov,

Hidetoshi Kubo, Kyoto University, kubo@cr.scphys.kyoto-u.ac.jp, 

Leonardo Di Venere, INFN Sezione di Bari, leonardo.divenere@ba.infn.it,

Lea Marcotulli, Clemson University, lmarcot@g.clemson.edu,

Jan Lommler, Die Johannes Gutenberg-Universität Mainz, lommler@uni-mainz.de, 

Lucas Parker, Los Alamos National Lab, lpp@lanl.gov, 

Luca Baldini, University of Pisa & INFN, luca.baldini@pi.infn.it,

Luca Foffano, University of Padova, luca.foffano@phd.unipd.it,

Luca Zampieri, Astronomical Observatory of Padova, luca.zampieri@oapd.inaf.it, 

Luigi Tibaldo, L'Observatoire Midi-Pyrénées, luigi.tibaldo@irap.omp.eu,

Maria Petropoulou, Princeton, m.petropoulou@astro.princeton.edu, 

Marco Ajello, Clemson University, majello@g.clemson.edu,

Manuel Meyer, Stanford University, mameyer@stanford.edu,

Marcos López, Universidad Complutense de Madrid, marcos@gae.ucm.es, 

Marc McConnell, University of New Hampshire, mark.mcconnell@unh.edu,

Markus Boettcher, North West University South Africa, Markus.Bottcher@nwu.ac.za, 

Martina Cardillo, Instituto Nazionale di Astrofisica, martina.cardillo@inaf.it, 

Manel Martinez, L'Institut de Física d'Altes Energies, martinez@ifae.es,

Matthew Kerr, Naval Research Lab, matthew.kerr@gmail.com,

M. Nicola Mazziotta, INFN Sezione di Bari, mazziotta@ba.infn.it,

Julie McEnery, NASA/GSFC, mcenery@milkyway.gsfc.nasa.gov,

Mattia Di Mauro, CRESST/NASA/GSFC, mdimauro@slac.stanford.edu,

Matthew Wood, SLAC National Accelerator Lab, mdwood@slac.stanford.edu,

Eileen Meyer, University of Maryland Baltimore County, meyer@umbc.edu,

Michael Briggs, University of Alabama Huntsville, michael.briggs@nasa.gov,

Michaël De Becker, Université de Liège, Michael.DeBecker@uliege.be,

Michael Lovellette, Naval Research Lab, michael.lovellette@nrl.navy.mil,

Michele Doro, University of Padova, michele.doro@unipd.it,

Miguel A. Sanchez-Conde, Universidad Autonoma de Madrid, miguel.sanchezconde@uam.es,

Michael Moss, George Washington University, mikejmoss3@gmail.com,

Tsunefumi Mizuno, Hiroshima University, mizuno@astro.hiroshima-u.ac.jp,

Marc Ribó, Universitat de Barcelona, mribo@fqa.ub.edu,

Kazuhiro Nakazawa, Nagoya University, nakazawa@u.phys.nagoya-u.ac.jp,

Naoko Kurahashi Neilson, Drexel University, naoko@icecube.wisc.edu,

Natalia Auricchio, INAF OAS Bologna, natalia.auricchio@inaf.it, 

Nicola Omodei, Stanford University, nicola.omodei@stanford.edu,

Uwe Oberlack, Die Johannes Gutenberg-Universität Mainz, oberlack@uni-mainz.de, 

Masanori Ohno, Hiroshima University, ohno@astro.hiroshima-u.ac.jp,

Elena Orlando, Stanford University, orland.ele@gmail.com, 

Nepomuk Otte, Georgia Tech, otte@gatech.edu,

Paolo Coppi, Yale University, paolo.coppi@yale.edu,

Peter Bloser, Los Alamos National Lab, peter.bloser@unh.edu,

Haocheng Zhang, Purdue University, phitlip2007@gmail.com, 

Philippe Laurent, Commissariat á l'Energie Atomique, plaurent@cea.fr,

Martin Pohl, Universität Potsdam, pohlmadq@gmail.com,

Elisa Prandini, University of Padova & INFN Padova, prandini@pd.infn.it,

Peter Shawhan, University of Maryland College Park, pshawhan@umd.edu,

Regina Caputo, NASA/GSFC, regina.caputo@nasa.gov,

Riccardo Campana, Instituto Nazionale di Astrofisica, riccardo.campana@inaf.it,

Riccardo Rando, University of Padova & INFN Padova, riccardo.rando@pd.infn.it,

Richard Woolf, Naval Research Lab, richard.woolf@nrl.navy.mil,

Robert Johnson, University of California Santa Cruz, rjohnson@scipp.ucsc.edu,

Roberto Mignani, Instituto Nazionale di Astrofisica, roberto.mignani@inaf.it,

Roland Walter, Université de Genève, roland.walter@unige.ch,

Roopesh Ojha, CRESST/NASA/GSFC, roopesh.ojha@gmail.com,

Rui Curado da Silva, Universidade de Coimbra, rui.silva@coimbra.lip.pt, 

Stefano Dietrich, Institute of Atmospheric Sciences and Climate, s.dietrich@isac.cnr.it,

Stefan Funk, Friedrich-Alexander-Universität Erlangen-Nürnberg, s.funk@fau.de,

Silvia Zane, University College London, s.zane@ucl.ac.uk, 

Sonia Anton, Universidade de Aveiro, santon@ua.pt,

Sara Buson, Universität Würzburg Lehrstuhl für Astronomie, sara.buson@gmail.com,

Sara Cutini, INFN Sezione di Perugia, sara.cutini@pg.infn.it,

Pablo Saz Parkinson, University of Hong Kong, sazpark2@gmail.com,

Richard Schirato, Los Alamos National Lab, schirato@lanl.gov,

Sean Griffin, CRESST/NASA/GSFC, sean.griffin@nasa.gov,

S. Kaufmann, Universidad Autónoma de Chiapas, skaufmann13@googlemail.com,

Lukasz Stawarz, Jagiellonian University, stawarz@oa.uj.edu.pl,

Stefano Ciprini, ASI Space Science Data Center, stefano.ciprini.asdc@gmail.com,

Stefano Del Sordo, Instituto Nazionale di Astrofisica, stefano.delsordo@inaf.it,

Sam Jones, Los Alamos National Lab, swjones@lanl.gov,

Sylvain Guiriec, George Washington University, sylvain.guiriec@gmail.com,

Hiro Tajima, Nagoya University, tajima@isee.nagoya-u.ac.jp, 

Teddy Cheung, Naval Research Lab, teddy.cheung@nrl.navy.mil,

Lih-Sin The, Clemson University, tlihsin@g.clemson.edu,

Tonia Venters, NASA/GSFC, tonia.m.venters@nasa.gov,

Troy Porter, Stanford University, tporter@stanford.edu,

Tim Linden, Stockholm University, trlinden@gmail.com, 

Ulisses Barres, Centro Brasileiro de Pesquisas Físicas, ulisses@cbpf.br, 

Vaidehi S Paliya, Deutsches Elektronen-Synchrotron (DESY), vaidehi.s.paliya@gmail.com,

Vladimir Bozhilov, Sofia University, vbozhilov@phys.uni-sofia.bg, 

Tom Vestrand, Los Alamos National Lab, vestrand@lanl.gov,

Vincent Tatischeff, CSNSM/IN2P3, vincent.tatischeff@csnsm.in2p3.fr, 

Wenlei Chen, Washington University in St. Louis, wenleichen@wustl.edu,

Xilu Wang, University of Illinois, xwang107@illinois.edu,

Yasuyuki Tanaka, Hiroshima University, ytanaka@astro.hiroshima-u.ac.jp,

Lucas Uhm, NPP/NASA/GSFC, z.lucas.uhm@gmail.com,

Bing Zhang, University of Nevada Las Vegas, zhang@physics.unlv.edu,

Stephan Zimmer, Universität Innsbruck, zimmer@slac.stanford.edu, 

Andreas Zoglauer, University of California Berkeley, zog@ssl.berkeley.edu,

Zorawar Wadiasingh, NPP/NASA/GSFC, zwadiasingh@gmail.com

